Analysis of Invariance and Robustness via Invertibility of ReLU-Networks

Studying the invertibility of deep neural networks (DNNs) provides a principled approach to better understand the behavior of these powerful models. Despite being a promising diagnostic tool, a consistent theory on their invertibility is still lacking. We derive a theoretically motivated approach to explore the preimages of ReLU-layers and mechanisms affecting the stability of the inverse. Using the developed theory, we numerically show how this approach uncovers characteristic properties of the network.

==> texts/def_retrieval.tex <==
\begin{definition}(Retrieval, singleton preimages)\ \\
\label{def_retrieval}
Let $A\in\mathbb{R}^{m\times n}$ and $b\in\mathbb{R}^m$. Then, $(A,b)$ does retrieval under $\relu$ (or more general a pointwise activation $\phi:\mathbb{R}\to\mathbb{R}$) for the point $x\in\mathbb{R}^n$ if the preimage of $\relu(Ax+b)$ is a singleton.\\
\end{definition}


==> texts/notation.tex <==
The following notations will be used with respect to (feed forward) neural networks.
\begin{itemize}
\item Input: $x=x_0\in\mathbb{R}^d=\mathbb{R}^{d_0}$
\item Preactivations: $z_l=A_lx_{l-1}+b_l\in\mathbb{R}^{d_l},$ where
	\begin{itemize}
	\item $A_l\in\mathbb{R}^{d_{l-1}\times d_l}$ and
	\item $b_l\in\mathbb{R}^{d_l}.$
	\end{itemize}
\item Activation: $x_l = g(z_l)\in\mathbb{R}^{d_l},$ where $g:\mathbb{R}\to\mathbb{R}$ the pointwise applied activation function. If nothing else is said we will assume $g=\relu$.
\item Number of layers: $L\in\mathbb{N}$
\item The whole net: $F:\mathbb{R}^d\ni x\mapsto F(x):=z:=z_L\in\mathbb{R}^{d_L}=\mathbb{R}^D$
\end{itemize}

For $A\in\mathbb{R}^{m\times n}$ a matrix and $I\subset[m]$, $A|_I$ denotes the matrix consisting of the rows of $A$'s whoes index is in $I$. Analogously for vectors.

For a vector $y\in\mathbb{R}^m$ the expression $y>0$ can be used to describe the index set $\{i:y_i>0\}$. Analogously for $<,=,\le,\ge$.

Every matrix $A\in\mathbb{R}^{m\times n}$ with the rows $a_i$, $i=1,\dots,m$, is associated with the set $A=\{a_i\}_{i=1}^m$ and vice versa every finite sets in $\mathbb{R}^n$ with a matrix (obviously only possible up to permutation of the indexing).


==> texts/observations_about_the_biased_setting.tex <==
If we now consider the biased setting, $$\relu Ax+b,$$ with $A\in\mathbb{R}^{m\times n}$, $x\in\mathbb{R}^n$ and $b\in\mathbb{R}^m$,we can make the following observations.
\begin{enumerate}
\item
$$y=\relu Ax+b$$
results in the mixed system
$$A|_{y>0}x+b|_{y>0}=y|_{y>0},$$
$$A|_{y\le0}x+b|_{y\le0}\le0.$$
Therefore only if the inequalities result in a unique solution, within the nullspace of $A|_{y>0}$, $x$ is uniquely determinable (if existing).
\item
If $O\in\mathbb{R}^{\nu\times n}$ is an orthonormal basis for a space $V\cong\mathbb{R}^\nu$, $\nu\le n$ (e.g. $V=\sN(A|_{y>0})$). Then a system $$Ax+b\le0$$ is uniquely solvable in $V$ if and only if $$AO^TOx+b\le0$$ is uniquely solvable in $\mathbb{R}^\nu$.
For $\overline A = AO^T$ and $\overline x = Ox$ it is possible to just look at a systems of inequalities of the form $$\overline A\overline x + b\le0,$$ for a general $\overline x \in\mathbb{R}^\nu$.
\item
A system $Ax+b\le0$, $x\in\mathbb{R}^\nu$, has a unique solution if and only if $(A,b)$ contains a subset of rows which is omnidirectional for some point $p\in\mathbb{R}^\nu$ -- assuming it has a solution at all. (See Lemma~\ref{lemma_inequalities}.)
\item 
Saying there is an omnidirectional set for a point $p\in\mathbb{R}^\nu$ is equivalent to saying one has a set of hyperplanes of $\mathbb{R}^\nu$ intersection in $p$ whoes normal vectors form an omnidirectional set in $\mathbb{R}^\nu$. But since an omnidirectional set has at least $\nu+1$ elements, since it has to form at least a simplex (see Theorem~\ref{thm_convex_hull}), its existence requires that $\nu+1$ hyperplanes intersect in one point. This never happens unless explicitly constructed.
\end{enumerate}
The four observations above result in the conclusion that the probability of recovering the part of $x$ which is in $\sN(A|_{Ax+b>0})$, unless there explicitly scheme to construct this, is 0.


==> texts/proof_thm_retrieval.tex <==
\begin{proof} (Theorem~\ref{retUnderReLU}, Retrieval under $\relu$) \\
\underline{First case:} If $\dim M =n$ then one has a system of linear equations that determines $x$ uniquely.\\
\underline{Second case:} From $\dim M = \tilde n < n$ it follows that $\sN(A|_{Ax>0})\ne\{0\}$ therefore the only hope of retrieving all information about $x$ lies in the reconstruction of the information lost in the nullspace by analyzing the system of inequalities, i.e. $A|_{Ax\le0}x\le0.$ Since if $A|_{Ax\le0}x\le0$ also $A|_{Ax\le0}2x\le0$ the only uniquely determinable $x$ in the nullspace has to be $0$ in it. This is, by definition, only possible if $A$ is omnidirectional.
\end{proof}


==> texts/thm_retrieval.tex <==
\begin{theorem}(Retrieval under $\relu$) \label{retUnderReLU}\\
Let $A\in\mathbb{R}^{m\times n}$ then $A$ does retrieval under $\relu$ for a point $x\in\mathbb{R}^n$ if and only if
\begin{itemize}
\item eiter
$$\dim M = n,$$ where $M:=\mbox{span}\ (A|_{Ax>0}),$
\item or
$A|_{Ax\le0}$ is omnidirectional in $M^\perp.$
\end{itemize}
\end{theorem}

